Quantum simulation of FMO complex using one-parameter semigroup of generators

The application of open quantum systems in biological processes such as photosynthetic complexes has recently received renewed attention. In this paper, we introduce a quantum algorithm for simulation of Markovian dynamics of the Fenna-Matthew-Olson (FMO) complex that exists in photosynthesis using a "universal set" of a one-parameter semigroup of generators. We investigate the details of each generator that has been obtained from spectral decomposition of the Gorini-Kossakowski-Sudarshan (GKS) matrix by using linear combination and unitary conjugation. Also, we present a simple quantum circuit for the implementation of these generators.

==> re2.tex <==
@article{r1,
  title={Quantum biology},
  author={Lambert, Neill and Chen, Yueh-Nan and Cheng, Yuan-Chung and Li, Che-Ming and Chen, Guang-Yin and Nori, Franco},
  journal={Nature Physics},
  volume={9},
  number={1},
  pages={10},
  year={2013},
  publisher={Nature Publishing Group}
}

@book{r2,
  title={Modern Quantum Chemistry: Action of light and organic crystals},
  author={Sinano{\u{g}}lu, Oktay},
  year={1965},
  publisher={Academic Press}
}

@article{r3,
  title={Exciton migration in molecular crystals},
  author={Grover, M and Silbey, R},
  journal={J. Chem. Phys.},
  volume={54},
  number={11},
  pages={4843--4851},
  year={1971},
  publisher={AIP}
}

@article{pp1,
author = {Jonas, David},
year = {2003},
month = {02},
pages = {425-63},
title = {Two-Dimensional Femtosecond Spectroscopy},
volume = {54},
journal = {Annual review of physical chemistry},
doi = {10.1146/annurev.physchem.54.011002.103907}
}

@article{pp2,
author = {Mukamel, Shaul},
year = {2000},
month = {02},
pages = {691-729},
title = {Multidimensional Femtosecond Correlation Spectroscopies of Electronic and Vibrational Excitations},
volume = {51},
journal = {Annual review of physical chemistry},
doi = {10.1146/annurev.physchem.51.1.691}
}

@article{pp3,
author = {Khalil, M and Demirdöven, N and Tokmakoff, Andrei},
year = {2003},
month = {06},
pages = {},
title = {Coherent 2D IR Spectroscopy: Molecular Structure and Dynamics in Solution},
volume = {107},
journal = {Journal of Physical Chemistry A - J PHYS CHEM A},
doi = {10.1021/jp0219247}
}

@article{pp4,
author = {Tian, Peifang and Keusters, Dorine and Suzaki, Yoshifumi and S Warren, Warren},
year = {2003},
month = {07},
pages = {1553-5},
title = {Femtosecond Phase-Coherent Two-Dimensional Spectroscopy},
volume = {300},
journal = {Science (New York, N.Y.)},
doi = {10.1126/science.1083433}
}

@article{pp5,
author = {Brixner, Tobias and Mancal, Tomas and V Stiopkin, Igor and R Fleming, Graham},
year = {2004},
month = {10},
pages = {4221-36},
title = {Phase-stabilized Two-dimensional Electronic Spectroscopy},
volume = {121},
journal = {The Journal of chemical physics},
doi = {10.1063/1.1776112}
}

@article{pp6,
author = {Brixner, T and V Stiopkin, I and R Fleming, G},
year = {2004},
month = {05},
pages = {884-6},
title = {Tunable two-dimensional femtosecond spectroscopy},
volume = {29},
journal = {Optics letters},
doi = {10.1364/OL.29.000884}
}






 @article{r4,
  title={Influence of phonons on exciton transfer dynamics: comparison of the Redfield, F{\"o}rster, and modified Redfield equations},
  author={Yang, Mino and Fleming, Graham R},
  journal={J. Chem. Phys.},
  volume={282},
  number={1},
  pages={163--180},
  year={2002},
  publisher={Elsevier}
}

@article{r5,
  title={Energy-transfer dynamics in the LHCII complex of higher plants: modified redfield approach},
  author={Novoderezhkin, Vladimir I and Palacios, Miguel A and Van Amerongen, Herbert and Van Grondelle, Rienk},
  journal={J. Phys. Chem. B},
  volume={108},
  number={29},
  pages={10363--10375},
  year={2004},
  publisher={ACS Publications}
}

@article{r6,
  title={Multichromophoric F{\"o}rster resonance energy transfer},
  author={Jang, Seogjoo and Newton, Marshall D and Silbey, Robert J},
  journal={Phys. Rev. Lett. },
  volume={92},
  number={21},
  pages={218301},
  year={2004},
  publisher={APS}
}

@article{r7,
  title={Highly efficient energy excitation transfer in light-harvesting complexes: The fundamental role of noise-assisted transport},
  author={Caruso, Filippo and Chin, Alex W and Datta, Animesh and Huelga, Susana F and Plenio, Martin B},
  journal={J. Phys. Chem. B },
  volume={131},
  number={10},
  pages={09B612},
  year={2009},
  publisher={AIP}
}

@article{Feynmann,
  title={ Photon-blockade-induced Mott transitions
and X Y spin models in coupled cavity arrays.},
  author={R.P. Feynmann},
  journal={Int. J. Theoret. Phys.},
  volume={21},
  number={467},
  pages={00},
  year={1982},
  }


@article{aa1,
  title={ Quantum simulation.},
  author={Andreas Trabesinger},
  journal={Nature Physics.},
  volume={8},
  number={263},
  pages={00},
  year={2012},
  }



@article{aa2,
  title = {Quantum simulation},
  author = {Georgescu, I. M. and Ashhab, S. and Nori, Franco},
  journal = {Rev. Mod. Phys.},
  volume = {86},
  issue = {1},
  pages = {153--185},
  numpages = {33},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.86.153},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.86.153}
}












@article{r8,
  title={Simulating physics with computers},
  author={Feynman, Richard P},
  journal={Int. J. Theor. Phys.},
  volume={21},
  number={6-7},
  pages={467--488},
  year={1982},
  publisher={Springer}
}

@book{r9,
  title={The theory of open quantum systems},
  author={Breuer, Heinz-Peter and Petruccione, Francesco and others},
  year={2002},
  publisher={Oxford University Press on Demand}
}

@article{r10,
  title={Implementation of quantum maps by programmable quantum processors},
  author={Hillery, Mark and Ziman, M{\'a}rio and Bu{\v{z}}ek, Vladim{\'\i}r},
  journal={Phys. Rev. A},
  volume={66},
  number={4},
  pages={042302},
  year={2002},
  publisher={APS}
}

@article{r11,
  title={Universal simulation of Markovian quantum dynamics},
  author={Bacon, Dave and Childs, Andrew M and Chuang, Isaac L and Kempe, Julia and Leung, Debbie W and Zhou, Xinlan},
  journal={Phys. Rev. A},
  volume={64},
  number={6},
  pages={062302},
  year={2001},
  publisher={APS}
}

@article{r12,
  title={Description of quantum dynamics of open systems based on collision-like models},
  author={Ziman, M{\"a}rio and {\v{S}}telmachovi{\v{c}}, Peter and Bu{\v{z}}ek, Vladim{\'\i}r},
  journal={J. Open Syst. Inform. Dynam.},
  volume={12},
  number={1},
  pages={81--91},
  year={2005},
  publisher={Springer}
}

@article{r13,
  title={Simulation of Markovian quantum dynamics on quantum logic networks},
  author={Koniorczyk, Matyas and Buzek, Vladimir and Adam, Peter and Laszlo, Akos},
  journal={arXiv preprint quant-ph/0205008},
  year={2002}
}

@article{r14,
  title={Simulation of generators of Markovian dynamics on programmable quantum processors},
  author={Koniorczyk, M and Bu{\v{z}}ek, V and Adam, P},
  journal={J. Eur. Phys. D},
  volume={37},
  number={2},
  pages={275--281},
  year={2006},
  publisher={Springer}
}

@article{r15,
  title={Solovay-kitaev decomposition strategy for single-qubit channels},
  author={Wang, Dong-Sheng and Berry, Dominic W and de Oliveira, Marcos C and Sanders, Barry C},
  journal={Phys. Rev. Lett.},
  volume={111},
  number={13},
  pages={130504},
  year={2013},
  publisher={APS}
}

@article{r16,
  title = {Universal simulation of Markovian open quantum systems},
  author = {Sweke, Ryan and Sinayskiy, Ilya and Bernard, Denis and Petruccione, Francesco},
  journal = {Phys. Rev. A},
  volume = {91},
  issue = {6},
  pages = {062308},
  numpages = {13},
  year = {2015},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.91.062308},
}






@article{r17,
  title={Open quantum system parameters for light harvesting complexes from molecular dynamics},
  author={Wang, Xiaoqing and Ritschel, Gerhard and W{\"u}ster, Sebastian and Eisfeld, Alexander},
  journal={J. Phys. Chem. B},
  volume={17},
  number={38},
  pages={25629--25641},
  year={2015},
  publisher={Royal Society of Chemistry}
}

@article{r18,
  title={Efficient energy transfer in light-harvesting systems, III: The influence of the eighth bacteriochlorophyll on the dynamics and efficiency in FMO},
  author={Moix, Jeremy and Wu, Jianlan and Huo, Pengfei and Coker, David and Cao, Jianshu},
  journal={The Journal of Physical Chemistry Letters},
  volume={2},
  number={24},
  pages={3045--3052},
  year={2011},
  publisher={ACS Publications}
}



@article{rr18,
  title={Chain mapping approach of Hamiltonian for FMO complex using associated, generalized and exceptional Jacobi polynomials},
  author={Mahdian, MBAM and Arjmandi, MB and Marahem, F},
  journal={International Journal of Modern Physics B},
  volume={30},
  number={18},
  pages={1650107},
  year={2016},
  publisher={World Scientific}
}
}

@article{r19,
  title={Normal mode analysis of the spectral density of the Fenna--Matthews--Olson light-harvesting protein: how the protein dissipates the excess energy of excitons},
  author={Renger, Thomas and Klinger, Alexander and Steinecker, Florian and Schmidt am Busch, Marcel and Numata, Jorge and Müh, Frank},
  journal={J. Phys. Chem.
B},
  volume={116},
  number={50},
  pages={14565--14580},
  year={2012},
  publisher={ACS Publications}
}

@article{r20,
  title={Simulated two-dimensional electronic spectroscopy of the eight-bacteriochlorophyll FMO complex},
  author={Yeh, Shu-Hao and Kais, Sabre},
  journal={J. Phys. Chem.
},
  volume={141},
  number={23},
  pages={12B645\_1},
  year={2014},
  publisher={AIP}
}

@article{r21,
  title={Emulation of complex open quantum systems using superconducting qubits},
  author={Mostame, Sarah and Huh, Joonsuk and Kreisbeck, Christoph and Kerman, Andrew J and Fujita, Takatoshi and Eisfeld, Alexander and Aspuru-Guzik, Al{\'a}n},
  journal={J. Quantum Inf. Process.},
  volume={16},
  number={2},
  pages={44},
  year={2017},
  publisher={Springer}
}

@article{r38,
  title={Highly efficient energy excitation transfer in light-harvesting complexes: The fundamental role of noise-assisted transport},
  author={Caruso, Filippo and Chin, Alex W and Datta, Animesh and Huelga, Susana F and Plenio, Martin B},
  journal={J. Chem. Phys.},
  volume={131},
  number={10},
  pages={09B612},
  year={2009},
  publisher={AIP}
}

@article{N11,
  title={Noise-assisted energy transfer in quantum networks and light-harvesting complexes},
  author={Chin, Alex W and Datta, Animesh and Caruso, Filippo and Huelga, Susana F and Plenio, Martin B},
  journal={New Journal of Physics},
  volume={12},
  number={6},
  pages={065002},
  year={2010},
  publisher={IOP Publishing}
}


@article{qs1,
  title={Efficient quantum simulation of photosynthetic light harvesting},
  author={Bi-Xue, Wang and Ming-Jie, Tao and Ai, Qing and Xin, Tao and Lambert, Neill and Ruan, Dong and Yuan-Chung, Cheng and Nori, Franco and Fu-Guo, Deng and Gui-Lu, Long},
  journal={NPJ Quantum Information},
  volume={4},
  pages={1--6},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{qs2,
  title={Quantum simulation of Fenna-Matthew-Olson (FMO) complex on a nuclear magnetic resonance (NMR) quantum computer},
  author={Mahdian, M and Yeganeh, H Davoodi},
  journal={arXiv preprint arXiv:1901.03118},
  year={2019}
}



@article{r22,
  title={On the product of semi-groups of operators},
  author={Trotter, Hale F},
  journal={Proc. Am. Math.
Soc},
  volume={10},
  number={4},
  pages={545--551},
  year={1959},
  publisher={JSTOR}
}
@article{f1,
  title={Quantum entanglement in photosynthetic light-harvesting complexes},
  author={Sarovar, Mohan and Ishizaki, Akihito and Fleming, Graham R and Whaley, K Birgitta},
  journal={Nature Physics},
  volume={6},
  number={6},
  pages={462--467},
  year={2010},
  publisher={Nature Publishing Group}
}
@article{f2,
  title={Entanglement and entangling power of the dynamics in light-harvesting complexes},
  author={Caruso, Filippo and Chin, Alex W and Datta, Animesh and Huelga, Susana F and Plenio, Martin B},
  journal={Physical Review A},
  volume={81},
  number={6},
  pages={062346},
  year={2010},
  publisher={APS}
}
@article{f3,
  title={Evidence for wavelike energy transfer through quantum coherence in photosynthetic systems},
  author={Engel, Gregory S and Calhoun, Tessa R and Read, Elizabeth L and Ahn, Tae-Kyu and Man{\v{c}}al, Tom{\'a}{\v{s}} and Cheng, Yuan-Chung and Blankenship, Robert E and Fleming, Graham R},
  journal={Nature},
  volume={446},
  number={7137},
  pages={782--786},
  year={2007},
  publisher={Nature Publishing Group}
}
@article{f4,
  title={Why quantum coherence is not important in the Fenna--Matthews--Olsen complex},
  author={Wilkins, David M and Dattani, Nikesh S},
  journal={Journal of chemical theory and computation},
  volume={11},
  number={7},
  pages={3411--3419},
  year={2015},
  publisher={ACS Publications}
}
@article{f5,
  title={Identification and characterization of diverse coherences in the Fenna--Matthews--Olson complex},
  author={Thyrhaug, Erling and Tempelaar, Roel and Alcocer, Marcelo JP and {\v{Z}}{\'\i}dek, Karel and B{\'\i}na, David and Knoester, Jasper and Jansen, Thomas LC and Zigmantas, Donatas},
  journal={Nature chemistry},
  volume={10},
  number={7},
  pages={780--786},
  year={2018},
  publisher={Nature Publishing Group}
}
@article{f6,
  title={Vibrational beatings conceal evidence of electronic coherence in the FMO light-harvesting complex},
  author={Tempelaar, Roel and Jansen, Thomas LC and Knoester, Jasper},
  journal={The Journal of Physical Chemistry B},
  volume={118},
  number={45},
  pages={12865--12872},
  year={2014},
  publisher={ACS Publications}
}

